ASAM: Boosting Segment Anything Model with Adversarial Tuning

In the evolving landscape of computer vision, foundation models have emerged as pivotal tools, exhibiting exceptional adaptability to a myriad of tasks. Among these, the Segment Anything Model (SAM) by Meta AI has distinguished itself in image segmentation. However, SAM, like its counterparts, encounters limitations in specific niche applications, prompting a quest for enhancement strategies that do not compromise its inherent capabilities. This paper introduces ASAM, a novel methodology that amplifies SAM's performance through adversarial tuning. We harness the potential of natural adversarial examples, inspired by their successful implementation in natural language processing. By utilizing a stable diffusion model, we augment a subset (1%) of the SA-1B dataset, generating adversarial instances that are more representative of natural variations rather than conventional imperceptible perturbations. Our approach maintains the photorealism of adversarial examples and ensures alignment with original mask annotations, thereby preserving the integrity of the segmentation task. The fine-tuned ASAM demonstrates significant improvements across a diverse range of segmentation tasks without necessitating additional data or architectural modifications. The results of our extensive evaluations confirm that ASAM establishes new benchmarks in segmentation tasks, thereby contributing to the advancement of foundational models in computer vision. Our project page is in https://asam2024.github.io/.

==> sec/0_abstract.tex <==
\begin{abstract}
The ABSTRACT is to be in fully justified italicized text, at the top of the left-hand column, below the author and affiliation information.
Use the word ``Abstract'' as the title, in 12-point Times, boldface type, centered relative to the column, initially capitalized.
The abstract is to be in 10-point, single-spaced type.
Leave two blank lines after the Abstract, then begin the main text.
Look at previous \confName abstracts to get a feel for style and length.
\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}
The concept of foundation models has been pivotal in advancing the fields of natural language processing (NLP) and, more recently, computer vision. Originating in NLP with influential models such as BERT~\cite{DBLP:conf/naacl/DevlinCLT19}, the GPT series~\cite{DBLP:journals/corr/abs-2303-08774}, and PaLM~\cite{DBLP:journals/jmlr/ChowdheryNDBMRBCSGSSTMRBTSPRDHPBAI23}, these models have showcased remarkable zero-shot generalization capabilities to unseen tasks. This success has spurred the development of similar paradigm-shifting models in computer vision.
These visual foundation models, such as DINOv2~\cite{DBLP:journals/corr/abs-2304-07193}, CLIP~\cite{DBLP:conf/icml/RadfordKHRGASAM21}, SAM~\cite{Kirillov_2023_ICCV,} and Stable Diffusion~\cite{DBLP:conf/cvpr/RombachBLEO22,}, demonstrate remarkable zero-shot capabilities and broad generalization across various tasks.

A prime example is the Segment Anything Model (SAM), a foundational vision model specializing in image segmentation, which has revolutionized the field with its ability to segment a diverse range of objects and structures across various scenarios.

Among these, the Segment Anything Model (SAM) stands out as a foundational vision model, specifically for image segmentation.

Recent years have witnessed the rise of foundation models in natural language processing (NLP), such as BERT, GPT-3, and PaLM. These large pretrained models have achieved state-of-the-art performance across diverse NLP tasks. Inspired by their success, the computer vision community has also developed powerful visual foundation models, including DALL-E, GLIDE, and SAM.

Among them, Segment Anything (SAM) stands out as a pioneering visual segmentation foundation model. Trained on over 1 billion masks from a massive visual corpus, SAM demonstrates strong zero-shot segmentation capabilities and generalizability. However, like other foundation models designed based on massive generic data, SAM may still struggle or underperform on certain niche downstream tasks.

The concept of foundation models, initially rooted in the field of natural language processing (NLP), has recently been extended to revolutionize the realm of computer vision. In NLP, models like BERT and GPT demonstrated the immense potential of these large-scale, versatile models, trained on extensive datasets to achieve unparalleled adaptability across a wide range of tasks. This paradigm shift, characterized by significant strides in representation learning, has spurred the exploration of task-agnostic models, propelling research into both their adaptation methodologies and the intricacies of their internal mechanisms.

In computer vision, this transformative trend is exemplified by the development of foundational vision models. These models, trained on diverse and expansive datasets, have shown remarkable capabilities in generating meaningful representations across multiple domains. The emergence of foundation models like DINO, CLIP, and BLIP has marked a significant departure from the traditional reliance on ImageNet-pretrained models, showcasing strong generalization across various tasks and settings




SAM, trained with billion-scale mask labels, has redefined image segmentation by demonstrating the ability to segment a diverse range of objects, parts, and visual structures in various scenarios. Its prompt-based approach and zero-shot segmentation abilities have led to a significant paradigm shift in the field, enabling rapid transfer to numerous applications with minimal input. Despite its impressive performance, SAM, like any foundational model, has areas where it can be further enhanced. Specifically, SAM faces challenges with coarse mask boundaries and incorrect predictions in complex scenarios, highlighting the need for models that can produce highly accurate segmentation masks without sacrificing zero-shot capabilities and operational efficiency



Trained on a vast scale with over a billion mask labels, SAM represents a significant stride in the field of computer vision. Its zero-shot segmentation abilities and prompt-based approach have facilitated rapid application across multiple domains \cite{63}. However, despite its impressive capabilities, SAM exhibits limitations in handling complex segmentation scenarios, often struggling with coarse mask boundaries and incorrect predictions \cite{63}.

Efforts to enhance SAM's performance have typically followed two routes. The first involves fine-tuning or using adapters for specific downstream tasks, which, while improving performance in those areas, often diminishes the model's generalization ability. The second approach preserves SAM's original parameters, adding adaptation layers or post-processing modules like in SAM-HQ. This method, though effective, requires additional parameters and annotated training data, limiting its scalability and efficiency \cite{64,65}.

These challenges bring us to the core motivation of our work: How can we improve the generalization ability of SAM as a foundational vision model without incurring high training costs, adding extra data, altering its structure, or compromising its zero-shot capabilities? Existing solutions, while effective in specific contexts, do not address the fundamental challenge of enhancing SAM's inherent performance across a diverse range of scenarios.

In response to this challenge, our approach draws inspiration from the realm of NLP, where adversarial training techniques have been successfully used not only to enhance model robustness but also to improve generalization. Unlike traditional adversarial training in the visual domain, which often leads to a trade-off between adversarial robustness and model performance, NLP techniques like FreeLB have shown that it's possible to achieve both robustness and improved generalization without additional computational costs. By applying a similar philosophy to SAM, our method aims to use "natural" adversarial examples, akin to those used in NLP, for training visual models. This approach promises to enhance SAM's segmentation accuracy and robustness while maintaining its foundational architecture and efficiency \cite{78,86,89}.

Thus, we propose a novel method that utilizes adversarial fine-tuning, inspired by the success of NLP adversarial training, to augment a portion of the SA-1B dataset with natural adversarial examples. This approach not only maintains the foundational traits of SAM but also marks a significant advancement in its capability to handle diverse segmentation tasks, setting a new precedent for cost-effective enhancements to foundational models in computer vision \cite{67}.






To address these problem, we propose a novel fine-tuning framework for large vision model called Photorealism-based Adversarial Tuning (PRAT).
Within this framework, we make the assumption that natural images can be projected onto a low-dimensional manifold through a generative model. 
Through training on natural images, this low-dimensional manifold ensures the photorealism and richness of content within the images. 
By mapping an image onto this manifold, shifting it along the adversarial direction on the manifold produces an natural and photorealitic adversarial example. 
In order to ensure that the object shape in the adversarial sample is consistent with the original mask label, during the process of mapping the manifold back to the image, we add an additional mask prompt branch in the generative model.
Finally, we utilized naturally realistic and accurately aligned adversarial examples, along with the original mask labels, to fine-tune a few subset of parameters in a large vision model, resulting in significant performance improvements.

==> sec/1_intro_rule.tex <==
\section{Introduction}
\label{sec:intro}

Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use options of \texttt{cvpr.sty} to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for readers to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
For your results, however, you should not identify yourself and should not mention your participation in the challenge.
Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.
\subsection{Segment Anything Model}\subsection{Segment Anything Model}
\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}


==> sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/3_related.tex <==
\section{Related Work}
\subsection{Segment Anything Model}
\subsection{Adversarial Training}

==> sec/4_method.tex <==
\section{Method}
\begin{figure*}
    \centering
    \includegraphics[width=0.9\textwidth]{CVPR2024-SAMADV/fig/pipline.pdf}
    \caption{Caption}
    \label{fig:enter-label} 
\end{figure*}
\subsection{Overview}
We intend to enhance the generalization performance of the Segment Anything Model (SAM) without depending on downstream datasets or making any architectural modifications to the model. To obtain accurate gradient updates for SAM, we perform a search for adversarial samples using the original SAM-1B dataset as a source.Initially, we apply the Image Latent Mapping (ILM) technique to map images onto a low-dimensional manifold, which represents the latent space. This captures the essential features and variations in a compressed representation.Subsequently, we introduce the Controlable Adversarial Latent Optimization (CALO) technique, which involves moving the latent representations of images along the adversarial direction on the manifold. This controlled manipulation allows us to generate adversarial samples challenging the SAM model.Finally, utilizing these adversarial latent representations, we generate corresponding adversarial images. Through a 'slow start, fast decay' learning rate schedule, we fine-tune the pre-trained SAM model. This process enables the model to adapt and learn from the adversarial variations present in the latent space, ultimately enhancing its generalization performance on unseen data.

\subsection{Adversarial Latent Generation}
For the diffusion model, the easiest image mapping is the inverse process of DDIM sampling [6, 43] with the condition embedding $C = \psi(P)$ of prompts P, based on the assumption that the ordinary differential equation (ODE) process can be reversed in the limit of small steps:
\begin{align}
    \mathcal{z}_{t+1} = \sqrt{\frac{\alpha_{t+1}}{\alpha_{t}}}\mathbf{z}_t + (\sqrt{\frac{1}{\alpha_{t+1}}-1} - \sqrt{\frac{1}{\alpha_t-1}}) \cdot \epsilon_\theta(\mathbf{z}_t,t,\mathcal{C}),
\end{align}
where $z_0$ is the given real image, a schedule $\left\{\beta_0,...,\beta_T \right\} \in (0, 1)$ and $\alpha_t=\prod_{1}^{t} (1-\beta_i)$.
In general, this process is the reverse direction of the denoising process ($z_0 \rightarrow z_T$ instead of $z_T 
\rightarrow z_0$), which can map the image $z_0$ to $z_T$ in the latent space. Image prompts are automatically generated using image caption models (e.g., BLIP v2 [27]). For simplicity, the encoding of the VAE is ignored.

Text-to-image synthesis usually emphasizes the effect of the prompt. Therefore, a classifier-free guidance technique [16] is proposed. Its prediction is also performed unconditionally, which is then extrapolated with the conditioned prediction. Given w as the guidance scale parameter and $
\emptyset = \psi(””)$ as the embedding of a null text, the classifier-free guidance prediction is expressed by:
\begin{align}
    \Tilde{\epsilon_\theta}(z_t,t,\mathbf{C},\emptyset) = \omega \cdot \epsilon_\theta(z_t,t,\mathbf{c}) + (1-\omega) \cdot \epsilon_\theta(z_t,t,\emptyset),
\end{align}
where $ \omega = 7.5$ is the default value for Stable Diffusion.
However, since the noise is predicted by the model $\epsilon_theta$ in the inverse process of DDIM sampling, a slight error is incorporated in every step.
Due to the existence of a large guidance scale parameter w in the classifier-free guidance technique, slight errors are amplified and lead to cumulative errors.
Consequently, executing the inverse process of DDIM sampling with classifier-free guidance not only disrupts the Gaussian distribution of noises but also induces visual artifacts of unreality [32].

To mitigate cumulative errors, we follw [32] and optimize a null text embedding $\emptyset_t$ for each timestamp $t$. First, the inverse process of DDIM sampling with $\omega = 1$ outputs a series of consecutive latents ${z_0^* , ..., z_T^* }$ where $z_0^* = z_0$.
Then, we conduct the following optimization with $\omega = 7.5$ (the default value for Stable Diffusion) and $ \bar{z}_T = z_t$ during N iterations for the timestamps $t = \left\{T, ..., 1 \right\}$:
\begin{align}
    \underset{\emptyset_t}{min} || z_(t-1)^* - z_{t-1}(\bar{z},t,\mathcal{C},\empty_t)  ||_2^2  
\end{align}

\begin{align}
    \begin{split} 
    z_(t-1)^* - z_{t-1}(\bar{z},t,\mathcal{C},\empty_t) = \sqrt{\frac{\alpha_(t-1)}{\alpha_t}}\bar{z}_t + \\(\sqrt{\frac{1}{\alpha_(t-1)}-1} - \sqrt{\frac{1}{\alpha_(t)}-1}) \cdot \Tilde{\epsilon}_\theta(z_t,t,\mathcal{C},\emptyset_t).
    \end{split}
\end{align}
Note that compared to other strategies [9, 39, 23, 49], the current strategy is simple and effective and does not require fine-tuning to obtain high-quality image reconstruction. Next, we exploit this latent to generate unrestricted adversarial examples.

In this section, we propose an optimization method for latents to maximize the attack performance on unrestricted adversarial examples. In the latent space of a given image after ILM, the null text embedding $\emptyset_t$ ensures the quality of the reconstructed image, while the text embedding $\mathcal{C}$ ensures the semantic information of the image.
Therefore, optimizing both embeddings may not be ideal. Considering that the noise  $\bar{z}_T$ largely represents the image’s information in the latent space, we choose to optimize it instead. However, this optimization is still challenged by complex gradient calculations and the overflow of the value range.
Based on the latents generated by ILM, we define the denoising process of diffusion models as $\emptyset(·)$ through Eqution 5, and it involves $T$ iterations:
\begin{align*}
    \begin{split}
    \Omega(z_t,T,\mathcal{C},\left\{\empty_t \right\}_1^T) = z_0(z_1(...,(z_(T-1),T- \\ 1,\mathcal{C},\emptyset_{T-1}),...,1,\mathcal{C},\emptyset_1),0,\mathcal{C},\emptyset_0)
    \end{split}
\end{align*}

Therefore, the reconstructed image is denoted as  $ \bar{z}_0 = \emptyset(z_T , T, C, \left\{\emptyset_t\right\})$. The computational process of VAE is disregarded herein, as it is differentiable. Combining Eqution 7, our adversarial objective optimization is expressed by:
\begin{align}
    \begin{split}
    \underset{max}{\delta} \mathcal{L}(\mathcal{F}_\theta(\bar{z_0}),y), s.t.||\delta||_{\infty} \leq \\ \kappa, \bar{z_0} = \Omega(z_T+\theta,T,\mathcal{C},{\emptyset_t}) \ \text{and} \ \bar{z_0} \ \text{is natural},     
    \end{split}
\end{align}
where $\delta$ is the adversarial perturbation on the latent space. Here, loss function $\mathcal{L}$ consists of crossentropy loss and mean square error, i.e., $\mathcal 
{L} = \beta\mathcal{L}_{mse} + \gamma\mathcal{L}_{bce} $.

To ensure the consistency of $z_0$ and  $\bar{z_0}$, we assume that $\delta$ does not change the consistency when $\delta$ is extremely small, i.e., $||\delta||_{\infty} \leq \kappa$.
The crux pertains to determining the optimal $\delta$ that yields the maximum classification loss.

Analogous to conventional adversarial attacks, we employ gradient-based techniques to estimate $\delta$ through: $\delta \simeq \eta \nabla _{z_T} \mathcal{L} (\mathcal{F}_\theta(\bar{z_0}), y)$, where $\eta$ denotes the magnitude of perturbations that occur in the direction of the gradient.
To expand $\nabla_{z_T} \mathcal{L} (\mathcal{F}\theta( \bar{z_0}), y)$ by the chain rule, we can have these derivative terms as follows:
\begin{align}
    \nabla_{z_T}\mathcal{L}(\mathcal{F}_\theta(\bar{z_T}),y) = \frac{\partial \mathcal{L}}{\partial \bar{z_0}} \cdot  \frac{\partial \bar{z_0}}{\partial \bar{z_1}} \cdot  \frac{\partial \bar{z_1}}{\partial \bar{z_2}}  \cdots \frac{\partial \bar{z_{T-1}}}{\partial \bar{z_{T}}}
\end{align}

\textbf{Skip Gradient} After observing the items, we find that although each item is differentiable, it is not feasible to derive the entire calculation graph. First, we analyze the term $\frac{ \nabla\mathcal{L}} {\nabla \bar{z_0}}$, which represents the derivative of the SAN with respect to the reconstructed image  $\dots{z_0}$ and provides the adversarial gradient direction. Then, for $\frac{\nabla z_t}{\nabla z_{t+1}}$ , each calculation of the derivative represents the calculation of a backpropagation. Furthermore, a complete denoising process accumulates $T$ calculation graphs, resulting in memory overflow (similar phenomena are also found in [40]). Therefore, the gradient of the denoising process cannot be directly calculated.
Fortunately, we propose a skip gradient to approximate $\frac{\partial \mathcal{\bar{z_0}}}{\partial \bar{z_T}} \cdot = \frac{\partial \bar{z_0}}{\partial \bar{z_1}} \cdot  \frac{\partial \bar{z_1}}{\partial \bar{z_2}}  \cdots \frac{\partial \bar{z_{T-1}}}{\partial \bar{z_{T}}}$. 
Recalling the diffusion process, the denoising process aims to eliminate the Gaussian noise added in DDIM sampling [43, 6, 38]. DDIM samples $z_t$ at any arbitrary time step $t$ in a closed form using reparameterization trick:
\begin{align}
    z_t = \sqrt{\alpha_t}z_0 + \sqrt{1 - \alpha_t} \epsilon, \epsilon \in \mathcal{N}(0,\textit{I}).
\end{align}

Consequently, we perform a manipulation by rearranging Equation 9 to obtain $z_0 = \frac{1}{\sqrt{\alpha_t}} z_t -\sqrt{\frac{1-\alpha_t}{\alpha_t}} \epsilon$. Therefore, we further obtain $\frac{\partial z_0}{\partial z_t} = \frac{1}{\sqrt{\alpha_t}}$ .In Stable Diffusion, timestep $t$ is at most 1000, so $\underset{t \rightarrow1000}{lim}  \frac{\partial z_0}{ \partial z_t} = \underset{t \rightarrow 1000}{lim}  \frac{1} {\sqrt{\alpha_t}} \thickapprox 14.58$.

In summary, $\frac{\partial z_0}{\partial z_t}$ can be regarded as a constant $\rho$ and Equation 8 can be re-expressed as $\nabla_{z_T}\mathcal{L}(\mathcal{F}_\theta(\bar{z_T}),y) = \rho \frac{\partial \mathcal{L}}{\partial \bar{z_0}}$. In summary, skip gradients approximate the gradients of the denoising process while reducing the computation and memory usage.

\textbf{Differentiable Boundary Processing.} Since the diffusion model does not explicitly constrain the value range of  $\bar{z0}$, the modification of $z_T$ may cause the value range to be exceeded. So we introduce differentiable boundary processing $\varrho$ to solve this problem. $\varrho$ constrains the values outside $[0, 1]$ to the range of $[0, 1]$ and the specific implementation refers to.

% Next, we define $\prod$ as the projection of the adversarial perturbation $\delta$ onto $\kappa-ball$. We introduce momentum $g$ and express the optimization adversarial latents as:
% \begin{align}
%     g_k \xleftarrow{} \mu \cdot g_{k-1} + \frac{\nabla_{z_T}\mathcal{L}(\mathcal{F}_\theta(\varrho(\bar{z_0})),y)}{{||\nabla_{z_T}\mathcal{L}(\mathcal{F}_\theta(\varrho(\bar{z_0})),y)||_1}
% \end{align}

\subsection{Controllable Latent Image Mapping}
\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{CVPR2024-SAMADV/fig/controlnet.pdf}
    \caption{Caption}
    \label{fig:controlnet}
\end{figure}
After obtaining adversarial latent, we can perform a reverse diffusion process to obtain the final adversarial examples. However, when a slight disturbance is added to the original latent variables, the generated image shape may not align well with the mask label. This problem can be solved by trying to incorporate more accurate prompt in the diffusion model. However, the existing text prompt is limited in controlling the spatial shape of the image, because it is difficult to accurately describe the shape of objects using text. To compensate for the limitation of text prompt, we additionally trained an mask-to-image ControlNet.

ControlNet manipulates task-specific conditions of denoising U-Net to further control the overall behavior of the entire diffusion model. 
The denoising U-Net without ControlNet is shown in Fig\ref{fig:controlnet}-(a).
We lock all parameters in $\theta$ and then alone clone the encoder's parameters into a trainable copy $\theta_c$. 
The replicated $\theta_c$ is trained using the external mask condition $m$ . 
The original parameters and the new parameters are called "locked copies" and "trainable copies". The motivation for making such copies rather than training the original weights directly is to avoid overfitting when the dataset is small and maintain production-ready quality for large models learned from billions of images. 
Decoder is connected through a unique type of convolution layer called "zero convolution", that is, a $1 \times 1$ convolution layer with both weights and biases initialized with zeros. We denote the zero convolution operation as $Z(·;·)$ and use two instances of parameters $\left\{ \theta_{z1}, \theta_{z2} \right\}$ to form the ControlNet structure with
\begin{align}
    y_c = F (x; \theta) + Z(F (x + Z( c; \theta_{z1}) ); \theta_c); \theta_{z2})    
\end{align}
where $y_c$ becomes the output of the neural network block, as shown in Figure 2-(b).

Different from the previous fine-tuning method of changing the structure of the SAM model, we want to comprehensively improve the capabilities of the SAM model without changing the structure of the SAM model.

Finally, we found that using a small number of adversarial samples and just fine-tuning the output token can bring considerable performance improvements, see the experiment.


